Bridging Text and Image for Artist Style Transfer via Contrastive Learning

Image style transfer has attracted widespread attention in the past few years. Despite its remarkable results, it requires additional style images available as references, making it less flexible and inconvenient. Using text is the most natural way to describe the style. More importantly, text can describe implicit abstract styles, like styles of specific artists or art movements. In this paper, we propose a Contrastive Learning for Artistic Style Transfer (CLAST) that leverages advanced image-text encoders to control arbitrary style transfer. We introduce a supervised contrastive training strategy to effectively extract style descriptions from the image-text model (i.e., CLIP), which aligns stylization with the text description. To this end, we also propose a novel and efficient adaLN based state space models that explore style-content fusion. Finally, we achieve a text-driven image style transfer. Extensive experiments demonstrate that our approach outperforms the state-of-the-art methods in artistic style transfer. More importantly, it does not require online fine-tuning and can render a 512x512 image in 0.03s.

==> Section/03_Preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}

At the core of our proposed TeXt-driven image STyle transfer \net, there are two key components: CLIP~\cite{clip} and Contrastive representation learning~\cite{simclr}. In the following, we discuss how CLIP has been employed in this context in previous literature and how we use Contrastive representation learning to embed CLIP for artist-aware style transfer.

\noindent \textbf{StyleCLIP} StyleCLIP~\cite{styleclip} uses the text description only for arbitrary facial image editing, like adding a mustache or glasses. The idea is to combine the generative power of styleGAN~\cite{stylegan,stylegan2} with the semantic abstraction of CLIP~\cite{clip} to discover latent space attribute editing. StyleCLIP provides three options for achieving text-guided manipulation. The first two approaches directly optimize the CLIP-space distance between text and image, with dedicated models for desirable changes. Similar concepts are further developed by CLIPstyler~\cite{language_2}, which takes augmented texts with the same meaning to optimize the network to produce reasonable stylizations iteratively. Figure~\ref{fig:method_compare} shows both processes of StyleCLIP and CLIPstyler. Given the target text $t_s$, their common goal is to optimize the distance $\Delta T$ to the generated image in the Clip space. Their difference is that StyleCLIP learns the generated image $G(\omega)$ from the latent code $\omega$, while CLIPstyler learns the stylization process of $f(I_c)$ from the source image $I_c$.
%
The third approach disentangles the feature representation in the latent space to find the latent-code entries that induce both the image-space change and the global direction of the two text descriptions (source and target). 

\noindent \textbf{SimCLR} For text-driven style transfer, there is one key issue to address: `Is text rich enough to represent the key features?' Text can explicitly describe the desirable styles, like \textit{stormy night}, \textit{colorful oil painting}, but it usually represents more abstract styles, like the name of artists (\textit{Van Gogh}) or the name of art movements (\textit{Impressionism}), which do not describe visual styles. Both StyleCLIP and CLIPstyler rely on the power of CLIP that can capture the co-linearity between texts and images. However, when the text prompts are domain-specific and abstract, minimizing the distance between stylized results and text prompts in the CLIP does not guarantee consistent visual matches. For instance, \textit{Van Gogh} has many paintings created at different periods, and visual appearances differ a lot. To learn one distinct and recognizable artistic style of \textit{Van Gogh}, we need to collect lots of his paintings and learn the visual features that are carried through all his paintings. The study on Contrastive representations learning~\cite{simclr} provides an alternative to text-driven style transfer. Given artists' names ($t_s$) and their paintings $I_s$, our proposed model applies both image-guided and text-guided stylization, as $I^\mathcal{I}_{cs}$ and $I^\mathcal{T}_{cs}$. Then it projects them onto the CLIP space and clusters them into groups, hence enabling arbitrary text-driven image style transfer. In other words, we learn to maximize the prior estimation of text distribution on the CLIP space. As shown in Figure~\ref{fig:fig_ana_wiki}(d), by finding the principal direction, in which the text features are projected, maximizing the distance between different texts (i.e., the yellow arrow of style differences between \textit{Picasso} and \textit{Van Gogh}), we can learn the most distinct feature representation for each text. In the meantime, we use contrastive learning to minimize the distance between paired images (i.e., the in-group distances (green and orange dash circles) of paintings created by \textit{Picasso} and \textit{Van Gogh}). We describe this mathematically as,

\begin{small}
	\begin{equation} \tag*{(1)}
	\begin{matrix}
% 	\begin{split}
	\!\begin{aligned}
	L_{\text{MC}} &= min\Delta T - max \Delta D \\
	&=min\sum_{i=1, j=1}^{i=N,j=C} \big(E^{i,j}_I(I^\mathcal{T}_{cs}),~E^j_T(t_{s})\big) +\\ &~~~~min\sum_{i=1, j=1, k\ne i}^{i,k=N,j=C} \big(E^{i,j}_I(I^\mathcal{I}_{cs}),~E^{k,j}_I(I^\mathcal{T}_{cs})\big)
	\label{eq:Equation1}
	\end{aligned}
% 	\end{split}
	\end{matrix} 
	\end{equation}
\end{small}

\noindent Where $N$ and $C$ are the number of images and classes. Equation~\ref{eq:Equation1} minimizes the intra-class distance $\Delta T$ between paired text-guided images $I^\mathcal{T}_{cs}$ and texts $t_s$, while maximizing the inter-class distance $\Delta D$ between images from different classes. The maximization of inter-class distance is approximately equivalent to minimizing the inter-class distance between text-guided ($I^\mathcal{T}_{cs}$) and image-guided ($I^\mathcal{I}_{cs}$) images from the same class. 


